Enhancing Data-Assimilation in CFD using Graph Neural Networks

We present a novel machine learning approach for data assimilation applied in fluid mechanics, based on adjoint-optimization augmented by Graph Neural Networks (GNNs) models. We consider as baseline the Reynolds-Averaged Navier-Stokes (RANS) equations, where the unknown is the meanflow and a closure model based on the Reynolds-stress tensor is required for correctly computing the solution. An end-to-end process is cast; first, we train a GNN model for the closure term. Second, the GNN model is introduced in the training process of data assimilation, where the RANS equations act as a physics constraint for a consistent prediction. We obtain our results using direct numerical simulations based on a Finite Element Method (FEM) solver; a two-fold interface between the GNN model and the solver allows the GNN's predictions to be incorporated into post-processing steps of the FEM analysis. The proposed scheme provides an excellent reconstruction of the meanflow without any features selection; preliminary results show promising generalization properties over unseen flow configurations.

==> packages.tex <==
\usepackage{arxiv}
\usepackage{subfigure}
\usepackage{subeqnarray}
\usepackage{bigfoot} % verbatim in footnotes...
\usepackage{wrapfig}
\usepackage{epstopdf,epsfig}
\usepackage{color}
\usepackage{tabularx}
\usepackage{amssymb}
\usepackage{amsfonts}
\usepackage{units}

\RequirePackage[T1]{fontenc}
\RequirePackage{amsmath}
\RequirePackage{graphicx}
\RequirePackage{mathptmx}      % use Times fonts if available on your TeX system
\RequirePackage{flushend}
\RequirePackage{mathrsfs}
\RequirePackage{bm}
\RequirePackage{natbib}
% \RequirePackage{subcaption}
\RequirePackage{xcolor}
\RequirePackage{url}
\RequirePackage[colorlinks,citecolor=blue,urlcolor=blue,linkcolor=blue]{hyperref}

